On random coarsening and its applications

In this paper, we use the Poincare separation theorem for estimating the eigenvalues of the fine grid. We propose a randomized version of the algorithm where several different coarse grids are constructed thus leading to more comprehensive eigenvalue estimates. The proposed algorithm is suited for modern day multicore and distributed processing.

==> eigenvalue_estimates.tex <==
\section{Eigenvalue estimates}
Poincare separation theorem relates the eigenvalues of the coarse grid
with those of the fine grid. Since, the eigenvalues of coarse grid are
completely sandwitched between the eigenvalues of the fine grid,
eigenvalues of the coarse grid are suitable candidates for shifts
while estimating the eigenvalues of the fine grid. 


\begin{algorithm} 
\caption{Eigenvalue estimate using aggregation based coarse grid} \label{pseudocode_eigen}
\begin{algorithmic}
\STATE INPUT: $A$, $k$=number of eigenvalues required
\STATE OUTPUT: $\{\lambda_1, \lambda_2, \lambda_3, \dots \lambda_k\}$

\STATE Compute coarse grid matrix $A_c$ as follows
\[
(A_c)_{ij} = \sum_{k \in G_i} \sum_{l \in G_j} a_{kl}
\]
where $1 \le i, \ j \le N_c$, and $a_{kl}$ is the $(k,l)th$ entry of $A$.

Here $G_{i}=\text{part}^{-1}(i)$, where 
\[ 
\text{part}^{-1}(i) = \{ \, j \in [1,\, N] \enspace \mid \enspace 
\text{part}(j)=i\,\}
\]

where part is the array containing partitioning information of the
graph of the matrix.  A graph partitioner could be used to obtain the
part array \cite{kar}.

\STATE Extract $\{\mu_1, \mu_2, \mu_3, \dots \mu_k\}$ = eigenvalues($A_c$)

\FOR{$j$ = 1 to $k$} \STATE $\lambda_i$=eigenvalue($A$, 1 $\mu_i$) //
Here $1$ denotes number of eigenvalues required and $\mu_i$ is the
proposed shift
\ENDFOR

\end{algorithmic}
\end{algorithm}

Once the part array is known, the interpolation operator $P$ could be
constructed easily, with that the coarse grid is constructed as $A_c =
P^TAP$. Let $N_c$ be the number of such aggregates, then the
interpolation matrix $P$ is defined as follows
\begin{equation} \label{interp} P_{ij} =
  \begin{cases}
    1, &\text{if $i \in G_{j}$,}\\
    0, &\text{otherwise,}\\
  \end{cases}
\end{equation}
Here, $1 \le i \le N, \, 1 \le j \le N_c$, $N$ being the size of the
original coefficient matrix $A$.

Small eigenvalues are often more useful than any other eigenvalues but
to obtain this eigenvalue via coarse grid we need an interpolation
operator such that tr($A_c$) is minimal. This is hard to obtain in
practice, however, in certain special cases (finite difference
problems, for example) some combinatorial approach could be used to
obtain interpolation operators such that the trace is close to minimum.
But in the most general case one could combine such combinatorial approach 
with randomization. 

\begin{algorithm} 
\caption{Eigenvalue estimate using aggregation based coarse grid} \label{pseudocode_eigen}
\begin{algorithmic}
\STATE INPUT: $A$, $k$=number of eigenvalues required
\STATE OUTPUT: $\{\lambda_1, \lambda_2, \lambda_3, \dots \lambda_k\}$

\STATE Compute coarse grid matrix $A_c$ as follows
\[
(A_c)_{ij} = \sum_{k \in G_i} \sum_{l \in G_j} a_{kl}
\]
where $1 \le i, \ j \le N_c$, and $a_{kl}$ is the $(k,l)th$ entry of $A$.

Here $G_{i}=\text{part}^{-1}(i)$, where 
\[ 
\text{part}^{-1}(i) = \{ \, j \in [1,\, N] \enspace \mid \enspace 
\text{part}(j)=i\,\}
\]

where part is the array containing partitioning information of the
graph of the matrix.  A graph partitioner could be used to obtain the
part array \cite{kar}.

\STATE Extract $\{\mu_1, \mu_2, \mu_3, \dots \mu_k\}$ = eigenvalues($A_c$)

\FOR{$j$ = 1 to $k$} \STATE $\lambda_i$=eigenvalue($A$, $\mu_i$) // $\mu_i$ is the shift 
%Here $1$ denotes number of eigenvalues required and $\mu_i$ is the
%proposed shift
\ENDFOR

\end{algorithmic}
\end{algorithm}

In Algo (\ref{pseudocode_eigen_random}), we show a possible {\em parallel} randomized
version of the algorithm.

\begin{algorithm}
  \caption{Randomozed eigenvalue estimate using aggregation based
    coarse grid} \label{pseudocode_eigen_random}
\begin{algorithmic}
\STATE INPUT: $A$, $J$
\STATE OUTPUT: eigenvalues of $A$

\FOR{$i$ = 1 to $J$} \STATE // parallel for

\STATE $A^i_c = P^T_i A P_i$

\STATE Extract $\{\mu^i_1, \mu^i_2, \mu^i_3, \dots \mu^i_k\}$ = eigenvalues($A^i_c$)

\FOR{$j$ = 1 to $k$} \STATE $\lambda^{i}_j$=eigenvalue($A$, $\mu^i_j$) // $\mu^i_j$ is the shift
\ENDFOR
%Here $1$ denotes number of eigenvalues required and $\mu_i$ is the
%proposed shift
\ENDFOR

\STATE $\Lambda = \{ \mu^1_1, \mu^1_2, \mu^1_3, \dots \mu^1_k \} \cup \{\mu^2_1, \mu^2_2, \mu^2_3, \dots \mu^2_k \} \cup \dots \cup \{ \mu^J_1, \mu^J_2, \mu^J_3, \dots \mu^J_k\}$

\end{algorithmic}
\end{algorithm}



==> gershgorin_circles.tex <==
\section*{Gershgorin circles}

\begin{theorem}[Gershgorin, 1931]
  The eigenvalues of $A\in \mathbb{C}^{N \times N}$ lie in the union
  of the $N$ discs in the complex plane
  \begin{align*}
    D_i = \{ \, z \in \mathbb{C} : |z-a_{ii}| \leq
    \sum\limits_{j=1,\,i \neq j}^{N} |a_{ij}| \, \}, \quad i = 1,
    \dots, N.
  \end{align*}
\end{theorem}
Using Greshgorin theorem, some simple propoerties of diagonally
dominant matrices can be derived.
\begin{theorem}
  A strictly diagonally dominant M-matrix is non-singular.
\end{theorem}
\begin{proof}
  The proof is by contradiction. Let $\lambda=0$ be an eigen-value of
  $A$ and let $x$ be the corresponding eigen-vector. By Greshgorin
  theorem, there exists an integer $m$ such that $\lambda$ lies in the
  disc $| 0 - a_{mm} | \leq \sum\limits_{j \neq
    m}^{N}|a_{mj}|$. Since, $A$ is strictly diagonally dominant
  M-matrix, we have $| a_{mm} | > \sum\limits_{j \neq
    m}^{N}|a_{mj}|$. Thus, we have a contradiction.
\end{proof}

Let $\lambda_i$ denote an arbitrary eigenvalue of $A$.  The trace of
an $n \times n$ matrix $A$ is defined to be the sum of the elements on
the main diagonal of A i.e.,
\[ tr(A) = \sum_{i=1}^{n}a_{ii},\] If $f(x) = (x-\lambda_1)^{d_1}
\cdots (x-\lambda_k)^{d_k}$ is the characteristic polynomial of a
matrix $A$, then
\[ tr(A)=d_1\lambda_1+ \cdots + d_k\lambda_k. \] Obviously, when the
eigenvalues are simple, we have the following relation
\begin{align}
  \sum_{i=1}^{n}a_{ii} = \sum_{i=1}^{n}\lambda_{i}
\end{align}



\begin{figure}
  \caption{Gershgorin circles for sky 10$\times$10$\times$10}
  \label{gershgorin_sky10}
  \begin{center}
    \includegraphics[scale=0.2]{gershgorin_circles_sky10.pdf}
  \end{center}
\end{figure}


\begin{figure}
  \caption{Gershgorin circles for rand, N=1000}
  \label{gershgorin_rand1000}
  \begin{center}
    \includegraphics[scale=0.3]{gershgorin_circles_rand1000.pdf}
  \end{center}
\end{figure}


\begin{figure}
  \caption{Gershgorin circles for sherman4, N=1104}
  \label{gershgorin_rand1000}
  \begin{center}
    \includegraphics[scale=0.3]{gershgorin_circles_sherman4.pdf}
  \end{center}
\end{figure}



==> poincare_separates.tex <==
\section{Poincar\'e separates}
Here we will see how poincare separates eigenvalues of two grid. Let
$K^T$ denote the transpose of a matrix $K$ and let $I_k$ denote the
identity matrix of size $k$.
\begin{theorem}[Poincar\'e]\label{Th:poincare} 
  Let $A$ be a symmetric $n \times n$ matrix
  with eigenvalues $\lambda_1 \le \lambda_2 \le \dots \le \lambda_n $,
  and let $P$ be a semi-orthogonal $n \times k$ matrix with the
  property that $P^TP=I_k$. The eigenvalues $\mu_1 \le \mu_2 \le
  \cdots \le \mu_{n-k+i}$ of $P^TAP$ are separated by the eigenvalues of $A$ as follows
\begin{align}
  \lambda_i \le \mu_{i} \le \lambda_{n-k+i}.
\end{align}
\end{theorem}
\begin{theorem}\label{Th:poincare_cor1}
  If $A$ is a real symmetric $n \times n$ matrix with eigenvalues $\lambda_1 \le \lambda_2 \le \cdots \le \lambda_n$, then the following holds
\begin{align}
  \min_{P^TP=I_k} tr(P^TAP) &= \sum_{i=1}^{k}\lambda_i, \\
  \max_{P^TP=I_k} tr(P^TAP) &= \sum_{i=1}^{k}\lambda_{n-k+i}.
\end{align}
\end{theorem}
\begin{theorem}
  If $A$ is a real symmetric $n \times n$ matrix with eigenvalues $\lambda_1 \le \lambda_2 \le \cdots \le \lambda_n$, and if the following conditions are satisfied 
\vspace{-5mm}
\begin{packed_enum}
  \item $tr(P^TAP)$ is minimum and 
  \item $P^TAP$ has simple eigenvalues
\end{packed_enum}
then we have 
\[ \mu_i = \lambda_i, \quad 1 \le i \le k, \] where $\mu_1 \le
\mu_2 \le \cdots \le \mu_{k}$ are eigenvalues of $P^TAP$.
\end{theorem}
\begin{proof}
  Since $P^TAP$ has simple eigenvalues, we have $tr(P^TAP) =
  \sum_{i=1}^{k}\mu_i$. Also, from Theorem \ref{Th:poincare_cor1}
  above, we have
  \begin{align}\label{Eq:trace}
    tr(P^TAP) = \sum_{i=1}^{k}\lambda_i.
  \end{align}
  We shall prove the hypothesis by
  contradiction. From \ref{Th:poincare}, we have $\mu_i \ge
  \lambda_i$. Let there exist $j$, $1 \le j \le k$, such that $\mu_i >
  \lambda_i$, then get
\begin{align}
  tr(P^TAP) = \sum_{i=1}^{k}\mu_i > \sum_{i=1}^{k}\lambda_i
\end{align}
contradicting \eqref{Eq:trace}. Thus, we must have $\mu_i =
\lambda_i$. The proof is complete.
\end{proof}
The theorem above tells us that if we are able to find a matrix $P$ such 
that $tr(P^TAP)$ is minimum, then the first $k$ smallest eigenvalues 
of the matrix $A$ are simply the eigenvalues of the matrix $P^TAP$ provided 
$P^TAP$ has simple eigenvalues.
\begin{theorem}
  If $A$ is a real symmetric $n \times n$ matrix with eigenvalues $\lambda_1 \le \lambda_2 \le \cdots \le \lambda_n$, and if the following conditions are satisfied 
\vspace{-5mm}
\begin{packed_enum}
  \item $tr(P^TAP)$ is maximum and 
  \item $P^TAP$ has simple eigenvalues
\end{packed_enum}
then we have 
\[ \mu_i = \lambda_{n-k+i}, \quad 1 \le i \le k, \] where $\mu_1 \le
\mu_2 \le \cdots \le \mu_{k}$ are eigenvalues of $P^TAP$.
\end{theorem}
\begin{proof}
  Since $P^TAP$ has simple eigenvalues, we have $tr(P^TAP) =
  \sum_{i=1}^{k}\mu_i$. Also, from Theorem \ref{Th:poincare_cor1}
  above, we have
  \begin{align}\label{Eq:trace2}
    tr(P^TAP) = \sum_{i=1}^{k}\lambda_{n+i-k}.
  \end{align}
  We shall prove the hypothesis by
  contradiction. From \ref{Th:poincare}, we have $\mu_i \le
  \lambda_i$. Let there exist $j$, $1 \le j \le k$, such that $\mu_i <
  \lambda_i$, then we get
\begin{align}
  tr(P^TAP) = \sum_{i=1}^{k}\mu_i < \sum_{i=1}^{k}\lambda_i
\end{align}
contradicting \eqref{Eq:trace2}. Thus, we must have $\mu_i =
\lambda_i$. The proof is complete.
\end{proof}
The theorem above tells us that if we are able to find a matrix $P$ such 
that $tr(P^TAP)$ is maximum, then the $k$ largest eigenvalues 
of the matrix $A$ are simply the eigenvalues of the matrix $P^TAP$ provided 
$P^TAP$ has simple eigenvalues. Determining first $k$ smallest or $k$ largest 
eigenvalues of a matrix is of prime importance in many applications. However, for these 
results to be of any practical use, there are two questions that need to be answered 
\begin{enumerate}
\item When does $P^TAP$ has simple eigenvalues ?
\item How can we find the matrix $P$ such that $tr(P^TAP)$ is minimum ?
\end{enumerate}
In what follows, we try to answer these questions.
\begin{theorem}
  If $A$ has simple eigenvalues, then $P^TAP$ has simple eigenvalues.
\end{theorem}
\begin{proof}
Proof follows from Theorem \ref{Th:poincare}.
\end{proof}


\begin{figure}
  \caption{Poincare separates for sky 10$\times$10$\times$10}
  \label{poincare_sky10}
  \begin{center}
    \includegraphics[scale=0.3]{poincare_separates_sky10.pdf}
  \end{center}
\end{figure}



\begin{figure}
  \caption{Poincare separates for sky 10$\times$10$\times$10 zoomed}
  \label{poincare_sky10_zoom}
  \begin{center}
    \includegraphics[scale=0.3]{poincare_separates_sky10_zoom.pdf}
  \end{center}
\end{figure}


